On the Selection of Calculable Residual Generators for UAV Fault Diagnosis

Structural Analysis is an established method for Fault Detection and Identification (FDI) in large-scale systems, enabling the discovery of Analytical Redundancy Relations (ARRs) which serve as residual generators. However, most techniques used to enumerate ARRs do not specify the matching used to calculate each of those ARRs. This can result in non-implementable or unusable residual generators, in the presence of non-invertibilities in the equations involved or in lack of computational tools. In this paper, we propose a methodology which combines a priori and a posteriori information in order to reduce the time required to find implementable, usable residual generators of minimum cost. The method is applied to a fixed-wing Unmanned Aerial Vehicle (UAV) model.

==> figures/ex_am.tex <==
\begin{small}

\tabcolsep=0.11cm
\setlength\extrarowheight{2pt}
\noindent
%\begin{center}
	
\begin{tabularx}{\linewidth}{|lr|*{12}{X}@{\quad}|*{4}{X}|} \cline{3-18}
\multicolumn{1}{l}{} & & \multicolumn{16}{c|}{Variables} \\ \cline{3-18}

\multicolumn{1}{l}{} & & $\dot{u}$ & $u$ & $w$ & $q$ & $\theta$ & $\dot{w}$ & $\dot{q}$ & $\dot{\theta}$ & $\dot{h}$ & $d_{gr}$ & $h$ & $h_{gr}$ & $\delta_e$ & $\delta_t$ & $y_1$ & $y_2$ \\ \hline

\multirow{13}{*}{\begin{sideways}Constraints\end{sideways}}

& \multicolumn{1}{|r|}{$c_1$} & 1 & 1 & 1 & 1 & 1 &   &   &   &   &   &   &   & 1 & 1 &   &   \\ 
& \multicolumn{1}{|r|}{$c_2$} &   & 1 & 1 & 1 & 1 & 1 &   &   &   &   &   &   & 1 &   &   &   \\ 
& \multicolumn{1}{|r|}{$c_3$} &   & 1 & 1 & 1 &   &   & 1 &   &   &   &   &   & 1 &   &   &   \\ 
& \multicolumn{1}{|r|}{$c_4$} &   &   &   & 1 &   &   &   & 1 &   &   &   &   &   &   &   &   \\ 
& \multicolumn{1}{|r|}{$c_5$} &   & 1 & 1 &   & 1 &   &   &   & 1 &   &   &   &   &   &   &   \\ 
& \multicolumn{1}{|r|}{$c_6$} &   &   &   &   &   &   &   &   &   & 1 & 1 & 1 &   &   &   &   \\ 
& \multicolumn{1}{|r|}{$d_1$} & 1 & 1 &   &   &   &   &   &   &   &   &   &   &   &   &   &   \\ 
& \multicolumn{1}{|r|}{$d_2$} &   &   & 1 &   &   & 1 &   &   &   &   &   &   &   &   &   &   \\ 
& \multicolumn{1}{|r|}{$d_3$} &   &   &   & 1 &   &   & 1 &   &   &   &   &   &   &   &   &   \\ 
& \multicolumn{1}{|r|}{$d_4$} &   &   &   &   & 1 &   &   & 1 &   &   &   &   &   &   &   &   \\
& \multicolumn{1}{|r|}{$d_5$} &   &   &   &   &   &   &   &   & 1 &   & 1 &   &   &   &   &   \\
& \multicolumn{1}{|r|}{$m_1$} &   &   &   & 1 &   &   &   &   &   &   &   &   &   &   & 1 &   \\
& \multicolumn{1}{|r|}{$m_2$} &   &   &   &   & 1 &   &   &   &   &   &   &   &   &   &   & 1 \\ \hline
\end{tabularx}

%\end{center}
\end{small}

==> graph.tex <==
\begin{tikzpicture}[node distance = 2cm, bend angle=45, auto]
\tikzstyle{known_var}=[circle, thick,fill=gray]
\tikzstyle{unkno_var}=[circle, draw=black, thick]
\tikzstyle{constr}=[rectangle, fill=black, thick, minimum height=10mm, minimum width = 1mm]
%
\begin{scope}

\node [known_var] [](xm) {$x_m$};
\node [constr] (m1) [below of=xm,label=$m_1$] {}
	edge [] (xm);
\node [unkno_var] (x) [below of=m1] {$x$}
	edge [] (m1);
\node [constr] (c1) [right of=x, label=$c_1$] {}
	edge [pre] (x);
\node [unkno_var] [right of=c1](xdot) {$\dot{x}$}
	edge [pre] (c1);
\node [constr] [right of=xdot, label=$c_2$] (c2) {}
	edge [] (xdot);
\node [unkno_var] [right of=c2] (v) {$v$}
	edge [] (c2);
\node [constr] (c3) [right of=v, label=$c_3$] {}
	edge [pre] (v);
\node [unkno_var] [right of=c3] (vdot) {$\dot{v}$}
	edge [pre] (c3);
\node [constr] [below of=c2, label=$c_4$] (c4) {}
	edge [bend right] (vdot)
	edge [bend left] (x);

\end{scope}
%
\end{tikzpicture}

==> graphMatch.tex <==
\begin{tikzpicture}[node distance = 2cm, bend angle=45, auto]
\tikzstyle{known_var}=[circle, thick,fill=gray]
\tikzstyle{unkno_var}=[circle, draw=black, thick]
\tikzstyle{constr}=[rectangle, fill=black, thick, minimum height=10mm, minimum width = 1mm]
%
\begin{scope}

\node [known_var] [](xm) {$x_m$};
\node [constr] (m1) [below of=xm,label=$m_1$] {}
	edge [] (xm);
\node [unkno_var] (x) [below of=m1] {$x$}
	edge [ultra thick] (m1);
\node [constr] (c1) [right of=x, label=$c_1$] {}
	edge [pre] (x);
\node [unkno_var] [right of=c1](xdot) {$\dot{x}$}
	edge [pre,ultra thick] (c1);
\node [constr] [right of=xdot, label=$c_2$] (c2) {}
	edge [] (xdot);
\node [unkno_var] [right of=c2] (v) {$v$}
	edge [ultra thick] (c2);
\node [constr] (c3) [right of=v, label=$c_3$] {}
	edge [pre] (v);
\node [unkno_var] [right of=c3] (vdot) {$\dot{v}$}
	edge [pre] (c3);
\node [constr] [below of=c2, label=$c_4$] (c4) {}
	edge [bend right,ultra thick] (vdot)
	edge [bend left] (x);
\node [known_var] [above of=c3] (zeroC3) {\tiny{ZERO}}
	edge [] (c3);
\end{scope}
%
\end{tikzpicture}

==> ranking.tex <==
\begin{algorithmic}[1]
	\Procedure{Ranking}{$\mathbf{G(\mathcal{C},\mathcal{X},\mathcal{E})}$}
	\State $\mathcal{X}_K^0 = \mathcal{X}_K$
	\State $r = 1$ \Comment Set the current rank
	\Statex \Comment{Repeat until all possible matchings have been done}
	\While{ $\mathcal{X}_U \neq \emptyset \wedge \mathcal{X}_K^{r-1}\neq\emptyset$ }
		\Statex \Comment{Find constraints with only one unmatched variable}
		\For{ $\forall c_i \in \mathcal{C}_U$ }
			\State $\mathcal{X}_{U,i} = var_U(c_i)$
			\State $\mathcal{X}_{K,i} = var_K(c_i)$
			\If{ $|\mathcal{X}_{U,i}|=1 \wedge \mathcal{X}_{K,i}^r = \emptyset$ }
				\State $\mathcal{X}_{K}^r = \mathcal{X}_{K}^r \bigcup \mathcal{X}_{U,i}$
				\State $\mathcal{C}_K^r = \mathcal{C}_K^r \bigcup \left\{ c_i \right\}$
			\EndIf
		\EndFor
		
		\Statex \Comment{Find residual generators}
		\For{ $\forall c_i \in \left\{c_i : c_i \in \mathcal{C}_U \wedge var_U(c_i)= \emptyset  \right\}$ }
			\State $\mathcal{X}_{K,i} = var_K(c_i)$
			\If { $\mathcal{X}_{K,i}^r=\emptyset$ }
				\State $\mathcal{C}_K^r = \mathcal{C}_K^r \bigcup \left\{c_i \right\}$
				\State $\mathcal{R}^r = \mathcal{R}^r \bigcup \left\{c_i \right\}$
			\EndIf
		\EndFor
		
		\State $r=r+1$

	\EndWhile
	\EndProcedure
\end{algorithmic}
